Who Needs Decoders? Efficient Estimation of Sequence-level Attributes

State-of-the-art sequence-to-sequence models often require autoregressive decoding, which can be highly expensive. However, for some downstream tasks such as out-of-distribution (OOD) detection and resource allocation, the actual decoding output is not needed just a scalar attribute of this sequence. In these scenarios, where for example knowing the quality of a system's output to predict poor performance prevails over knowing the output itself, is it possible to bypass the autoregressive decoding? We propose Non-Autoregressive Proxy (NAP) models that can efficiently predict general scalar-valued sequence-level attributes. Importantly, NAPs predict these metrics directly from the encodings, avoiding the expensive autoregressive decoding stage. We consider two sequence-to-sequence task: Machine Translation (MT); and Automatic Speech Recognition (ASR). In OOD for MT, NAPs outperform a deep ensemble while being significantly faster. NAPs are also shown to be able to predict performance metrics such as BERTScore (MT) or word error rate (ASR). For downstream tasks, such as data filtering and resource optimization, NAPs generate performance predictions that outperform predictive uncertainty while being highly inference efficient.

==> tex/abstract_drafts.tex <==
% DRAFT 3

\begin{abstract}
    Many 
\end{abstract}


% DRAFT 2

\begin{abstract}
    State-of-the-art sequence-to-sequence models require autoregressive decoding, which grows expensive with sequence, model, and ensemble size.
    %
    However, upon decoding, many tasks such as OOD detection and resource allocation reduce the full output to a single estimate of information-theoretic or performance-based metrics.
    %
    The output is subsequently discarded.
    %
    In such scenarios, where knowing the quality of a model's output, and preempting poor performance, prevails over knowing the output itself, can we bypass full decoding?
    %
    We train Non-Autoregressive Proxy (NAP) models that can efficiently predict general scalar-valued sequence-level attributes produced by an autoregressive (T5) system, for both Neural Machine Translation and Automatic Speech Recognition.
    %
    Importantly, NAPs predict these metrics directly from encodings, without the use of an autoregressive decoder.
    %
    We use it to perform OOD detection in Machine Translation, significantly outperforming a deep ensemble while being 46-138x faster.
    %
    Furthermore, we train NAPs to directly predict performance metrics such as BERTScore of decoded outputs.
    %
    Predictions produced by these NAPs outperform model confidence and entropy in predicting poor performance.
    %
    This success was also found when predicting word error rates for Automatic Speech Recognition (using pretrained Whisper) models, in this case, 42x faster than full inference.
\end{abstract}



% ORIGINAL
\begin{abstract}
    Autoregressive decoding can be expensive, 
    % Mention seq2seq here
    % Mention scenarios here before mentioning bypassing at all
    but can we bypass it when the full decoded output is not required? 
    %
    In many scenarios, knowing the quality of a model's output, and preempting poor performance, prevails over knowing the output itself.
    %
    We train Non-Autoregressive Proxy (NAP) models that can efficiently directly predict general scalar-valued sequence-level attributes. % generated by an 
    % conditioned on an autoregressive model. 
    % 
    % Start here with the main split in applications: MT vs. ASR
    % Trained on information theoretic attributes of the seq2seq tasks, as well as performance-based metrics, such as ...
    Here, we investigate training NAP models to predict the confidence, entropy, or mutual information uncertainty produced by an autoregressive (T5) system.
    % 
    We use it to perform OOD detection in Machine Translation, significantly outperforming a deep ensemble while being 46-138x faster.
    %
    Furthermore, we train NAPs to directly predict performance metrics such as BERTScore of decoded outputs.
    %
    Predictions produced by these NAPs outperform model confidence and entropy in predicting poor performance.
    %
    This success was also found when predicting word error rates for Automatic Speech Recognition (using pretrained Whisper) models, in this case, 42x faster than full inference.
    % Faster than standard implementation of ...
    %
    % Finally, the above results are all achieved with a novel loss that only accounts for rank ordering of predictions.
\end{abstract}

